Evidence for the strangeness-changing weak decay $\Xi_b^-\to\Lambda_b^0\pi^-$

Using a $pp$ collision data sample corresponding to an integrated luminosity of 3.0~fb$^{-1}$, collected by the LHCb detector, we present the first search for the strangeness-changing weak decay $\Xi_b^-\to\Lambda_b^0\pi^-$. No $b$ hadron decay of this type has been seen before. A signal for this decay, corresponding to a significance of 3.2 standard deviations, is reported. The relative rate is measured to be ${{f_{\Xi_b^-}}\over{f_{\Lambda_b^0}}}{\cal{B}}(\Xi_b^-\to\Lambda_b^0\pi^-) = (5.7\pm1.8^{+0.8}_{-0.9})\times10^{-4}$, where $f_{\Xi_b^-}$ and $f_{\Lambda_b^0}$ are the $b\to\Xi_b^-$ and $b\to\Lambda_b^0$ fragmentation fractions, and ${\cal{B}}(\Xi_b^-\to\Lambda_b^0\pi^-)$ is the branching fraction. Assuming $f_{\Xi_b^-}/f_{\Lambda_b^0}$ is bounded between 0.1 and 0.3, the branching fraction ${\cal{B}}(\Xi_b^-\to\Lambda_b^0\pi^-)$ would lie in the range from $(0.57\pm0.21)\%$ to $(0.19\pm0.07)\%$.

==> LHCb_HD_authorlist_2015-08-17.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\centerline{\large\bf LHCb collaboration}
\begin{flushleft}
\small
R.~Aaij$^{38}$, 
C.~Abell\'{a}n~Beteta$^{40}$, 
B.~Adeva$^{37}$, 
M.~Adinolfi$^{46}$, 
A.~Affolder$^{52}$, 
Z.~Ajaltouni$^{5}$, 
S.~Akar$^{6}$, 
J.~Albrecht$^{9}$, 
F.~Alessio$^{38}$, 
M.~Alexander$^{51}$, 
S.~Ali$^{41}$, 
G.~Alkhazov$^{30}$, 
P.~Alvarez~Cartelle$^{53}$, 
A.A.~Alves~Jr$^{57}$, 
S.~Amato$^{2}$, 
S.~Amerio$^{22}$, 
Y.~Amhis$^{7}$, 
L.~An$^{3}$, 
L.~Anderlini$^{17}$, 
J.~Anderson$^{40}$, 
G.~Andreassi$^{39}$, 
M.~Andreotti$^{16,f}$, 
J.E.~Andrews$^{58}$, 
R.B.~Appleby$^{54}$, 
O.~Aquines~Gutierrez$^{10}$, 
F.~Archilli$^{38}$, 
P.~d'Argent$^{11}$, 
A.~Artamonov$^{35}$, 
M.~Artuso$^{59}$, 
E.~Aslanides$^{6}$, 
G.~Auriemma$^{25,m}$, 
M.~Baalouch$^{5}$, 
S.~Bachmann$^{11}$, 
J.J.~Back$^{48}$, 
A.~Badalov$^{36}$, 
C.~Baesso$^{60}$, 
W.~Baldini$^{16,38}$, 
R.J.~Barlow$^{54}$, 
C.~Barschel$^{38}$, 
S.~Barsuk$^{7}$, 
W.~Barter$^{38}$, 
V.~Batozskaya$^{28}$, 
V.~Battista$^{39}$, 
A.~Bay$^{39}$, 
L.~Beaucourt$^{4}$, 
J.~Beddow$^{51}$, 
F.~Bedeschi$^{23}$, 
I.~Bediaga$^{1}$, 
L.J.~Bel$^{41}$, 
V.~Bellee$^{39}$, 
N.~Belloli$^{20,j}$, 
I.~Belyaev$^{31}$, 
E.~Ben-Haim$^{8}$, 
G.~Bencivenni$^{18}$, 
S.~Benson$^{38}$, 
J.~Benton$^{46}$, 
A.~Berezhnoy$^{32}$, 
R.~Bernet$^{40}$, 
A.~Bertolin$^{22}$, 
M.-O.~Bettler$^{38}$, 
M.~van~Beuzekom$^{41}$, 
A.~Bien$^{11}$, 
S.~Bifani$^{45}$, 
P.~Billoir$^{8}$, 
T.~Bird$^{54}$, 
A.~Birnkraut$^{9}$, 
A.~Bizzeti$^{17,h}$, 
T.~Blake$^{48}$, 
F.~Blanc$^{39}$, 
J.~Blouw$^{10}$, 
S.~Blusk$^{59}$, 
V.~Bocci$^{25}$, 
A.~Bondar$^{34}$, 
N.~Bondar$^{30,38}$, 
W.~Bonivento$^{15}$, 
S.~Borghi$^{54}$, 
M.~Borisyak$^{65}$, 
M.~Borsato$^{7}$, 
T.J.V.~Bowcock$^{52}$, 
E.~Bowen$^{40}$, 
C.~Bozzi$^{16,38}$, 
S.~Braun$^{11}$, 
M.~Britsch$^{11}$, 
T.~Britton$^{59}$, 
J.~Brodzicka$^{54}$, 
N.H.~Brook$^{46}$, 
E.~Buchanan$^{46}$, 
C.~Burr$^{54}$, 
A.~Bursche$^{40}$, 
J.~Buytaert$^{38}$, 
S.~Cadeddu$^{15}$, 
R.~Calabrese$^{16,f}$, 
M.~Calvi$^{20,j}$, 
M.~Calvo~Gomez$^{36,o}$, 
P.~Campana$^{18}$, 
D.~Campora~Perez$^{38}$, 
L.~Capriotti$^{54}$, 
A.~Carbone$^{14,d}$, 
G.~Carboni$^{24,k}$, 
R.~Cardinale$^{19,i}$, 
A.~Cardini$^{15}$, 
P.~Carniti$^{20,j}$, 
L.~Carson$^{50}$, 
K.~Carvalho~Akiba$^{2,38}$, 
G.~Casse$^{52}$, 
L.~Cassina$^{20,j}$, 
L.~Castillo~Garcia$^{38}$, 
M.~Cattaneo$^{38}$, 
Ch.~Cauet$^{9}$, 
G.~Cavallero$^{19}$, 
R.~Cenci$^{23,s}$, 
M.~Charles$^{8}$, 
Ph.~Charpentier$^{38}$, 
M.~Chefdeville$^{4}$, 
S.~Chen$^{54}$, 
S.-F.~Cheung$^{55}$, 
N.~Chiapolini$^{40}$, 
M.~Chrzaszcz$^{40}$, 
X.~Cid~Vidal$^{38}$, 
G.~Ciezarek$^{41}$, 
P.E.L.~Clarke$^{50}$, 
M.~Clemencic$^{38}$, 
H.V.~Cliff$^{47}$, 
J.~Closier$^{38}$, 
V.~Coco$^{38}$, 
J.~Cogan$^{6}$, 
E.~Cogneras$^{5}$, 
V.~Cogoni$^{15,e}$, 
L.~Cojocariu$^{29}$, 
G.~Collazuol$^{22}$, 
P.~Collins$^{38}$, 
A.~Comerma-Montells$^{11}$, 
A.~Contu$^{15}$, 
A.~Cook$^{46}$, 
M.~Coombes$^{46}$, 
S.~Coquereau$^{8}$, 
G.~Corti$^{38}$, 
M.~Corvo$^{16,f}$, 
B.~Couturier$^{38}$, 
G.A.~Cowan$^{50}$, 
D.C.~Craik$^{48}$, 
A.~Crocombe$^{48}$, 
M.~Cruz~Torres$^{60}$, 
S.~Cunliffe$^{53}$, 
R.~Currie$^{53}$, 
C.~D'Ambrosio$^{38}$, 
E.~Dall'Occo$^{41}$, 
J.~Dalseno$^{46}$, 
P.N.Y.~David$^{41}$, 
A.~Davis$^{57}$, 
O.~De~Aguiar~Francisco$^{2}$, 
K.~De~Bruyn$^{6}$, 
S.~De~Capua$^{54}$, 
M.~De~Cian$^{11}$, 
J.M.~De~Miranda$^{1}$, 
L.~De~Paula$^{2}$, 
P.~De~Simone$^{18}$, 
C.-T.~Dean$^{51}$, 
D.~Decamp$^{4}$, 
M.~Deckenhoff$^{9}$, 
L.~Del~Buono$^{8}$, 
N.~D\'{e}l\'{e}age$^{4}$, 
M.~Demmer$^{9}$, 
D.~Derkach$^{65}$, 
O.~Deschamps$^{5}$, 
F.~Dettori$^{38}$, 
B.~Dey$^{21}$, 
A.~Di~Canto$^{38}$, 
F.~Di~Ruscio$^{24}$, 
H.~Dijkstra$^{38}$, 
S.~Donleavy$^{52}$, 
F.~Dordei$^{11}$, 
M.~Dorigo$^{39}$, 
A.~Dosil~Su\'{a}rez$^{37}$, 
D.~Dossett$^{48}$, 
A.~Dovbnya$^{43}$, 
K.~Dreimanis$^{52}$, 
L.~Dufour$^{41}$, 
G.~Dujany$^{54}$, 
P.~Durante$^{38}$, 
R.~Dzhelyadin$^{35}$, 
A.~Dziurda$^{26}$, 
A.~Dzyuba$^{30}$, 
S.~Easo$^{49,38}$, 
U.~Egede$^{53}$, 
V.~Egorychev$^{31}$, 
S.~Eidelman$^{34}$, 
S.~Eisenhardt$^{50}$, 
U.~Eitschberger$^{9}$, 
R.~Ekelhof$^{9}$, 
L.~Eklund$^{51}$, 
I.~El~Rifai$^{5}$, 
Ch.~Elsasser$^{40}$, 
S.~Ely$^{59}$, 
S.~Esen$^{11}$, 
H.M.~Evans$^{47}$, 
T.~Evans$^{55}$, 
A.~Falabella$^{14}$, 
C.~F\"{a}rber$^{38}$, 
N.~Farley$^{45}$, 
S.~Farry$^{52}$, 
R.~Fay$^{52}$, 
D.~Ferguson$^{50}$, 
V.~Fernandez~Albor$^{37}$, 
F.~Ferrari$^{14}$, 
F.~Ferreira~Rodrigues$^{1}$, 
M.~Ferro-Luzzi$^{38}$, 
S.~Filippov$^{33}$, 
M.~Fiore$^{16,38,f}$, 
M.~Fiorini$^{16,f}$, 
M.~Firlej$^{27}$, 
C.~Fitzpatrick$^{39}$, 
T.~Fiutowski$^{27}$, 
K.~Fohl$^{38}$, 
P.~Fol$^{53}$, 
M.~Fontana$^{15}$, 
F.~Fontanelli$^{19,i}$, 
D. C.~Forshaw$^{59}$, 
R.~Forty$^{38}$, 
M.~Frank$^{38}$, 
C.~Frei$^{38}$, 
M.~Frosini$^{17}$, 
J.~Fu$^{21}$, 
E.~Furfaro$^{24,k}$, 
A.~Gallas~Torreira$^{37}$, 
D.~Galli$^{14,d}$, 
S.~Gallorini$^{22}$, 
S.~Gambetta$^{50}$, 
M.~Gandelman$^{2}$, 
P.~Gandini$^{55}$, 
Y.~Gao$^{3}$, 
J.~Garc\'{i}a~Pardi\~{n}as$^{37}$, 
J.~Garra~Tico$^{47}$, 
L.~Garrido$^{36}$, 
D.~Gascon$^{36}$, 
C.~Gaspar$^{38}$, 
R.~Gauld$^{55}$, 
L.~Gavardi$^{9}$, 
G.~Gazzoni$^{5}$, 
D.~Gerick$^{11}$, 
E.~Gersabeck$^{11}$, 
M.~Gersabeck$^{54}$, 
T.~Gershon$^{48}$, 
Ph.~Ghez$^{4}$, 
S.~Gian\`{i}$^{39}$, 
V.~Gibson$^{47}$, 
O.G.~Girard$^{39}$, 
L.~Giubega$^{29}$, 
V.V.~Gligorov$^{38}$, 
C.~G\"{o}bel$^{60}$, 
D.~Golubkov$^{31}$, 
A.~Golutvin$^{53,38}$, 
A.~Gomes$^{1,a}$, 
C.~Gotti$^{20,j}$, 
M.~Grabalosa~G\'{a}ndara$^{5}$, 
R.~Graciani~Diaz$^{36}$, 
L.A.~Granado~Cardoso$^{38}$, 
E.~Graug\'{e}s$^{36}$, 
E.~Graverini$^{40}$, 
G.~Graziani$^{17}$, 
A.~Grecu$^{29}$, 
E.~Greening$^{55}$, 
S.~Gregson$^{47}$, 
P.~Griffith$^{45}$, 
L.~Grillo$^{11}$, 
O.~Gr\"{u}nberg$^{63}$, 
B.~Gui$^{59}$, 
E.~Gushchin$^{33}$, 
Yu.~Guz$^{35,38}$, 
T.~Gys$^{38}$, 
T.~Hadavizadeh$^{55}$, 
C.~Hadjivasiliou$^{59}$, 
G.~Haefeli$^{39}$, 
C.~Haen$^{38}$, 
S.C.~Haines$^{47}$, 
S.~Hall$^{53}$, 
B.~Hamilton$^{58}$, 
X.~Han$^{11}$, 
S.~Hansmann-Menzemer$^{11}$, 
N.~Harnew$^{55}$, 
S.T.~Harnew$^{46}$, 
J.~Harrison$^{54}$, 
J.~He$^{38}$, 
T.~Head$^{39}$, 
V.~Heijne$^{41}$, 
K.~Hennessy$^{52}$, 
P.~Henrard$^{5}$, 
L.~Henry$^{8}$, 
E.~van~Herwijnen$^{38}$, 
M.~He\ss$^{63}$, 
A.~Hicheur$^{2}$, 
D.~Hill$^{55}$, 
M.~Hoballah$^{5}$, 
C.~Hombach$^{54}$, 
W.~Hulsbergen$^{41}$, 
T.~Humair$^{53}$, 
N.~Hussain$^{55}$, 
D.~Hutchcroft$^{52}$, 
D.~Hynds$^{51}$, 
M.~Idzik$^{27}$, 
P.~Ilten$^{56}$, 
R.~Jacobsson$^{38}$, 
A.~Jaeger$^{11}$, 
J.~Jalocha$^{55}$, 
E.~Jans$^{41}$, 
A.~Jawahery$^{58}$, 
M.~John$^{55}$, 
D.~Johnson$^{38}$, 
C.R.~Jones$^{47}$, 
C.~Joram$^{38}$, 
B.~Jost$^{38}$, 
N.~Jurik$^{59}$, 
S.~Kandybei$^{43}$, 
W.~Kanso$^{6}$, 
M.~Karacson$^{38}$, 
T.M.~Karbach$^{38,\dagger}$, 
S.~Karodia$^{51}$, 
M.~Kecke$^{11}$, 
M.~Kelsey$^{59}$, 
I.R.~Kenyon$^{45}$, 
M.~Kenzie$^{38}$, 
T.~Ketel$^{42}$, 
E.~Khairullin$^{65}$, 
B.~Khanji$^{20,38,j}$, 
C.~Khurewathanakul$^{39}$, 
S.~Klaver$^{54}$, 
K.~Klimaszewski$^{28}$, 
O.~Kochebina$^{7}$, 
M.~Kolpin$^{11}$, 
I.~Komarov$^{39}$, 
R.F.~Koopman$^{42}$, 
P.~Koppenburg$^{41,38}$, 
M.~Kozeiha$^{5}$, 
L.~Kravchuk$^{33}$, 
K.~Kreplin$^{11}$, 
M.~Kreps$^{48}$, 
G.~Krocker$^{11}$, 
P.~Krokovny$^{34}$, 
F.~Kruse$^{9}$, 
W.~Krzemien$^{28}$, 
W.~Kucewicz$^{26,n}$, 
M.~Kucharczyk$^{26}$, 
V.~Kudryavtsev$^{34}$, 
A. K.~Kuonen$^{39}$, 
K.~Kurek$^{28}$, 
T.~Kvaratskheliya$^{31}$, 
D.~Lacarrere$^{38}$, 
G.~Lafferty$^{54,38}$, 
A.~Lai$^{15}$, 
D.~Lambert$^{50}$, 
G.~Lanfranchi$^{18}$, 
C.~Langenbruch$^{48}$, 
B.~Langhans$^{38}$, 
T.~Latham$^{48}$, 
C.~Lazzeroni$^{45}$, 
R.~Le~Gac$^{6}$, 
J.~van~Leerdam$^{41}$, 
J.-P.~Lees$^{4}$, 
R.~Lef\`{e}vre$^{5}$, 
A.~Leflat$^{32,38}$, 
J.~Lefran\c{c}ois$^{7}$, 
E.~Lemos~Cid$^{37}$, 
O.~Leroy$^{6}$, 
T.~Lesiak$^{26}$, 
B.~Leverington$^{11}$, 
Y.~Li$^{7}$, 
T.~Likhomanenko$^{65,64}$, 
M.~Liles$^{52}$, 
R.~Lindner$^{38}$, 
C.~Linn$^{38}$, 
F.~Lionetto$^{40}$, 
B.~Liu$^{15}$, 
X.~Liu$^{3}$, 
D.~Loh$^{48}$, 
I.~Longstaff$^{51}$, 
J.H.~Lopes$^{2}$, 
D.~Lucchesi$^{22,q}$, 
M.~Lucio~Martinez$^{37}$, 
H.~Luo$^{50}$, 
A.~Lupato$^{22}$, 
E.~Luppi$^{16,f}$, 
O.~Lupton$^{55}$, 
A.~Lusiani$^{23}$, 
F.~Machefert$^{7}$, 
F.~Maciuc$^{29}$, 
O.~Maev$^{30}$, 
K.~Maguire$^{54}$, 
S.~Malde$^{55}$, 
A.~Malinin$^{64}$, 
G.~Manca$^{7}$, 
G.~Mancinelli$^{6}$, 
P.~Manning$^{59}$, 
A.~Mapelli$^{38}$, 
J.~Maratas$^{5}$, 
J.F.~Marchand$^{4}$, 
U.~Marconi$^{14}$, 
C.~Marin~Benito$^{36}$, 
P.~Marino$^{23,38,s}$, 
J.~Marks$^{11}$, 
G.~Martellotti$^{25}$, 
M.~Martin$^{6}$, 
M.~Martinelli$^{39}$, 
D.~Martinez~Santos$^{37}$, 
F.~Martinez~Vidal$^{66}$, 
D.~Martins~Tostes$^{2}$, 
A.~Massafferri$^{1}$, 
R.~Matev$^{38}$, 
A.~Mathad$^{48}$, 
Z.~Mathe$^{38}$, 
C.~Matteuzzi$^{20}$, 
A.~Mauri$^{40}$, 
B.~Maurin$^{39}$, 
A.~Mazurov$^{45}$, 
M.~McCann$^{53}$, 
J.~McCarthy$^{45}$, 
A.~McNab$^{54}$, 
R.~McNulty$^{12}$, 
B.~Meadows$^{57}$, 
F.~Meier$^{9}$, 
M.~Meissner$^{11}$, 
D.~Melnychuk$^{28}$, 
M.~Merk$^{41}$, 
E~Michielin$^{22}$, 
D.A.~Milanes$^{62}$, 
M.-N.~Minard$^{4}$, 
D.S.~Mitzel$^{11}$, 
J.~Molina~Rodriguez$^{60}$, 
I.A.~Monroy$^{62}$, 
S.~Monteil$^{5}$, 
M.~Morandin$^{22}$, 
P.~Morawski$^{27}$, 
A.~Mord\`{a}$^{6}$, 
M.J.~Morello$^{23,s}$, 
J.~Moron$^{27}$, 
A.B.~Morris$^{50}$, 
R.~Mountain$^{59}$, 
F.~Muheim$^{50}$, 
D.~M\"{u}ller$^{54}$, 
J.~M\"{u}ller$^{9}$, 
K.~M\"{u}ller$^{40}$, 
V.~M\"{u}ller$^{9}$, 
M.~Mussini$^{14}$, 
B.~Muster$^{39}$, 
P.~Naik$^{46}$, 
T.~Nakada$^{39}$, 
R.~Nandakumar$^{49}$, 
A.~Nandi$^{55}$, 
I.~Nasteva$^{2}$, 
M.~Needham$^{50}$, 
N.~Neri$^{21}$, 
S.~Neubert$^{11}$, 
N.~Neufeld$^{38}$, 
M.~Neuner$^{11}$, 
A.D.~Nguyen$^{39}$, 
T.D.~Nguyen$^{39}$, 
C.~Nguyen-Mau$^{39,p}$, 
V.~Niess$^{5}$, 
R.~Niet$^{9}$, 
N.~Nikitin$^{32}$, 
T.~Nikodem$^{11}$, 
A.~Novoselov$^{35}$, 
D.P.~O'Hanlon$^{48}$, 
A.~Oblakowska-Mucha$^{27}$, 
V.~Obraztsov$^{35}$, 
S.~Ogilvy$^{51}$, 
O.~Okhrimenko$^{44}$, 
R.~Oldeman$^{15,e}$, 
C.J.G.~Onderwater$^{67}$, 
B.~Osorio~Rodrigues$^{1}$, 
J.M.~Otalora~Goicochea$^{2}$, 
A.~Otto$^{38}$, 
P.~Owen$^{53}$, 
A.~Oyanguren$^{66}$, 
A.~Palano$^{13,c}$, 
F.~Palombo$^{21,t}$, 
M.~Palutan$^{18}$, 
J.~Panman$^{38}$, 
A.~Papanestis$^{49}$, 
M.~Pappagallo$^{51}$, 
L.L.~Pappalardo$^{16,f}$, 
C.~Pappenheimer$^{57}$, 
W.~Parker$^{58}$, 
C.~Parkes$^{54}$, 
G.~Passaleva$^{17}$, 
G.D.~Patel$^{52}$, 
M.~Patel$^{53}$, 
C.~Patrignani$^{19,i}$, 
A.~Pearce$^{54,49}$, 
A.~Pellegrino$^{41}$, 
G.~Penso$^{25,l}$, 
M.~Pepe~Altarelli$^{38}$, 
S.~Perazzini$^{14,d}$, 
P.~Perret$^{5}$, 
L.~Pescatore$^{45}$, 
K.~Petridis$^{46}$, 
A.~Petrolini$^{19,i}$, 
M.~Petruzzo$^{21}$, 
E.~Picatoste~Olloqui$^{36}$, 
B.~Pietrzyk$^{4}$, 
T.~Pila\v{r}$^{48}$, 
D.~Pinci$^{25}$, 
A.~Pistone$^{19}$, 
A.~Piucci$^{11}$, 
S.~Playfer$^{50}$, 
M.~Plo~Casasus$^{37}$, 
T.~Poikela$^{38}$, 
F.~Polci$^{8}$, 
A.~Poluektov$^{48,34}$, 
I.~Polyakov$^{31}$, 
E.~Polycarpo$^{2}$, 
A.~Popov$^{35}$, 
D.~Popov$^{10,38}$, 
B.~Popovici$^{29}$, 
C.~Potterat$^{2}$, 
E.~Price$^{46}$, 
J.D.~Price$^{52}$, 
J.~Prisciandaro$^{37}$, 
A.~Pritchard$^{52}$, 
C.~Prouve$^{46}$, 
V.~Pugatch$^{44}$, 
A.~Puig~Navarro$^{39}$, 
G.~Punzi$^{23,r}$, 
W.~Qian$^{4}$, 
R.~Quagliani$^{7,46}$, 
B.~Rachwal$^{26}$, 
J.H.~Rademacker$^{46}$, 
M.~Rama$^{23}$, 
M.~Ramos~Pernas$^{37}$, 
M.S.~Rangel$^{2}$, 
I.~Raniuk$^{43}$, 
N.~Rauschmayr$^{38}$, 
G.~Raven$^{42}$, 
F.~Redi$^{53}$, 
S.~Reichert$^{54}$, 
M.M.~Reid$^{48}$, 
A.C.~dos~Reis$^{1}$, 
S.~Ricciardi$^{49}$, 
S.~Richards$^{46}$, 
M.~Rihl$^{38}$, 
K.~Rinnert$^{52,38}$, 
V.~Rives~Molina$^{36}$, 
P.~Robbe$^{7,38}$, 
A.B.~Rodrigues$^{1}$, 
E.~Rodrigues$^{54}$, 
J.A.~Rodriguez~Lopez$^{62}$, 
P.~Rodriguez~Perez$^{54}$, 
S.~Roiser$^{38}$, 
V.~Romanovsky$^{35}$, 
A.~Romero~Vidal$^{37}$, 
J. W.~Ronayne$^{12}$, 
M.~Rotondo$^{22}$, 
T.~Ruf$^{38}$, 
P.~Ruiz~Valls$^{66}$, 
J.J.~Saborido~Silva$^{37}$, 
N.~Sagidova$^{30}$, 
P.~Sail$^{51}$, 
B.~Saitta$^{15,e}$, 
V.~Salustino~Guimaraes$^{2}$, 
C.~Sanchez~Mayordomo$^{66}$, 
B.~Sanmartin~Sedes$^{37}$, 
R.~Santacesaria$^{25}$, 
C.~Santamarina~Rios$^{37}$, 
M.~Santimaria$^{18}$, 
E.~Santovetti$^{24,k}$, 
A.~Sarti$^{18,l}$, 
C.~Satriano$^{25,m}$, 
A.~Satta$^{24}$, 
D.M.~Saunders$^{46}$, 
D.~Savrina$^{31,32}$, 
M.~Schiller$^{38}$, 
H.~Schindler$^{38}$, 
M.~Schlupp$^{9}$, 
M.~Schmelling$^{10}$, 
T.~Schmelzer$^{9}$, 
B.~Schmidt$^{38}$, 
O.~Schneider$^{39}$, 
A.~Schopper$^{38}$, 
M.~Schubiger$^{39}$, 
M.-H.~Schune$^{7}$, 
R.~Schwemmer$^{38}$, 
B.~Sciascia$^{18}$, 
A.~Sciubba$^{25,l}$, 
A.~Semennikov$^{31}$, 
N.~Serra$^{40}$, 
J.~Serrano$^{6}$, 
L.~Sestini$^{22}$, 
P.~Seyfert$^{20}$, 
M.~Shapkin$^{35}$, 
I.~Shapoval$^{16,43,f}$, 
Y.~Shcheglov$^{30}$, 
T.~Shears$^{52}$, 
L.~Shekhtman$^{34}$, 
V.~Shevchenko$^{64}$, 
A.~Shires$^{9}$, 
B.G.~Siddi$^{16}$, 
R.~Silva~Coutinho$^{40}$, 
L.~Silva~de~Oliveira$^{2}$, 
G.~Simi$^{22}$, 
M.~Sirendi$^{47}$, 
N.~Skidmore$^{46}$, 
T.~Skwarnicki$^{59}$, 
E.~Smith$^{55,49}$, 
E.~Smith$^{53}$, 
I.T.~Smith$^{50}$, 
J.~Smith$^{47}$, 
M.~Smith$^{54}$, 
H.~Snoek$^{41}$, 
M.D.~Sokoloff$^{57,38}$, 
F.J.P.~Soler$^{51}$, 
F.~Soomro$^{39}$, 
D.~Souza$^{46}$, 
B.~Souza~De~Paula$^{2}$, 
B.~Spaan$^{9}$, 
P.~Spradlin$^{51}$, 
S.~Sridharan$^{38}$, 
F.~Stagni$^{38}$, 
M.~Stahl$^{11}$, 
S.~Stahl$^{38}$, 
S.~Stefkova$^{53}$, 
O.~Steinkamp$^{40}$, 
O.~Stenyakin$^{35}$, 
S.~Stevenson$^{55}$, 
S.~Stoica$^{29}$, 
S.~Stone$^{59}$, 
B.~Storaci$^{40}$, 
S.~Stracka$^{23,s}$, 
M.~Straticiuc$^{29}$, 
U.~Straumann$^{40}$, 
L.~Sun$^{57}$, 
W.~Sutcliffe$^{53}$, 
K.~Swientek$^{27}$, 
S.~Swientek$^{9}$, 
V.~Syropoulos$^{42}$, 
M.~Szczekowski$^{28}$, 
T.~Szumlak$^{27}$, 
S.~T'Jampens$^{4}$, 
A.~Tayduganov$^{6}$, 
T.~Tekampe$^{9}$, 
M.~Teklishyn$^{7}$, 
G.~Tellarini$^{16,f}$, 
F.~Teubert$^{38}$, 
C.~Thomas$^{55}$, 
E.~Thomas$^{38}$, 
J.~van~Tilburg$^{41}$, 
V.~Tisserand$^{4}$, 
M.~Tobin$^{39}$, 
J.~Todd$^{57}$, 
S.~Tolk$^{42}$, 
L.~Tomassetti$^{16,f}$, 
D.~Tonelli$^{38}$, 
S.~Topp-Joergensen$^{55}$, 
N.~Torr$^{55}$, 
E.~Tournefier$^{4}$, 
S.~Tourneur$^{39}$, 
K.~Trabelsi$^{39}$, 
M.T.~Tran$^{39}$, 
M.~Tresch$^{40}$, 
A.~Trisovic$^{38}$, 
A.~Tsaregorodtsev$^{6}$, 
P.~Tsopelas$^{41}$, 
N.~Tuning$^{41,38}$, 
A.~Ukleja$^{28}$, 
A.~Ustyuzhanin$^{65,64}$, 
U.~Uwer$^{11}$, 
C.~Vacca$^{15,38,e}$, 
V.~Vagnoni$^{14}$, 
G.~Valenti$^{14}$, 
A.~Vallier$^{7}$, 
R.~Vazquez~Gomez$^{18}$, 
P.~Vazquez~Regueiro$^{37}$, 
C.~V\'{a}zquez~Sierra$^{37}$, 
S.~Vecchi$^{16}$, 
J.J.~Velthuis$^{46}$, 
M.~Veltri$^{17,g}$, 
G.~Veneziano$^{39}$, 
M.~Vesterinen$^{11}$, 
B.~Viaud$^{7}$, 
D.~Vieira$^{2}$, 
M.~Vieites~Diaz$^{37}$, 
X.~Vilasis-Cardona$^{36,o}$, 
V.~Volkov$^{32}$, 
A.~Vollhardt$^{40}$, 
D.~Volyanskyy$^{10}$, 
D.~Voong$^{46}$, 
A.~Vorobyev$^{30}$, 
V.~Vorobyev$^{34}$, 
C.~Vo\ss$^{63}$, 
J.A.~de~Vries$^{41}$, 
R.~Waldi$^{63}$, 
C.~Wallace$^{48}$, 
R.~Wallace$^{12}$, 
J.~Walsh$^{23}$, 
S.~Wandernoth$^{11}$, 
J.~Wang$^{59}$, 
D.R.~Ward$^{47}$, 
N.K.~Watson$^{45}$, 
D.~Websdale$^{53}$, 
A.~Weiden$^{40}$, 
M.~Whitehead$^{48}$, 
G.~Wilkinson$^{55,38}$, 
M.~Wilkinson$^{59}$, 
M.~Williams$^{38}$, 
M.P.~Williams$^{45}$, 
M.~Williams$^{56}$, 
T.~Williams$^{45}$, 
F.F.~Wilson$^{49}$, 
J.~Wimberley$^{58}$, 
J.~Wishahi$^{9}$, 
W.~Wislicki$^{28}$, 
M.~Witek$^{26}$, 
G.~Wormser$^{7}$, 
S.A.~Wotton$^{47}$, 
S.~Wright$^{47}$, 
K.~Wyllie$^{38}$, 
Y.~Xie$^{61}$, 
Z.~Xu$^{39}$, 
Z.~Yang$^{3}$, 
J.~Yu$^{61}$, 
X.~Yuan$^{34}$, 
O.~Yushchenko$^{35}$, 
M.~Zangoli$^{14}$, 
M.~Zavertyaev$^{10,b}$, 
L.~Zhang$^{3}$, 
Y.~Zhang$^{3}$, 
A.~Zhelezov$^{11}$, 
A.~Zhokhov$^{31}$, 
L.~Zhong$^{3}$, 
S.~Zucchelli$^{14}$.\bigskip

{\footnotesize \it
$ ^{1}$Centro Brasileiro de Pesquisas F\'{i}sicas (CBPF), Rio de Janeiro, Brazil\\
$ ^{2}$Universidade Federal do Rio de Janeiro (UFRJ), Rio de Janeiro, Brazil\\
$ ^{3}$Center for High Energy Physics, Tsinghua University, Beijing, China\\
$ ^{4}$LAPP, Universit\'{e} Savoie Mont-Blanc, CNRS/IN2P3, Annecy-Le-Vieux, France\\
$ ^{5}$Clermont Universit\'{e}, Universit\'{e} Blaise Pascal, CNRS/IN2P3, LPC, Clermont-Ferrand, France\\
$ ^{6}$CPPM, Aix-Marseille Universit\'{e}, CNRS/IN2P3, Marseille, France\\
$ ^{7}$LAL, Universit\'{e} Paris-Sud, CNRS/IN2P3, Orsay, France\\
$ ^{8}$LPNHE, Universit\'{e} Pierre et Marie Curie, Universit\'{e} Paris Diderot, CNRS/IN2P3, Paris, France\\
$ ^{9}$Fakult\"{a}t Physik, Technische Universit\"{a}t Dortmund, Dortmund, Germany\\
$ ^{10}$Max-Planck-Institut f\"{u}r Kernphysik (MPIK), Heidelberg, Germany\\
$ ^{11}$Physikalisches Institut, Ruprecht-Karls-Universit\"{a}t Heidelberg, Heidelberg, Germany\\
$ ^{12}$School of Physics, University College Dublin, Dublin, Ireland\\
$ ^{13}$Sezione INFN di Bari, Bari, Italy\\
$ ^{14}$Sezione INFN di Bologna, Bologna, Italy\\
$ ^{15}$Sezione INFN di Cagliari, Cagliari, Italy\\
$ ^{16}$Sezione INFN di Ferrara, Ferrara, Italy\\
$ ^{17}$Sezione INFN di Firenze, Firenze, Italy\\
$ ^{18}$Laboratori Nazionali dell'INFN di Frascati, Frascati, Italy\\
$ ^{19}$Sezione INFN di Genova, Genova, Italy\\
$ ^{20}$Sezione INFN di Milano Bicocca, Milano, Italy\\
$ ^{21}$Sezione INFN di Milano, Milano, Italy\\
$ ^{22}$Sezione INFN di Padova, Padova, Italy\\
$ ^{23}$Sezione INFN di Pisa, Pisa, Italy\\
$ ^{24}$Sezione INFN di Roma Tor Vergata, Roma, Italy\\
$ ^{25}$Sezione INFN di Roma La Sapienza, Roma, Italy\\
$ ^{26}$Henryk Niewodniczanski Institute of Nuclear Physics  Polish Academy of Sciences, Krak\'{o}w, Poland\\
$ ^{27}$AGH - University of Science and Technology, Faculty of Physics and Applied Computer Science, Krak\'{o}w, Poland\\
$ ^{28}$National Center for Nuclear Research (NCBJ), Warsaw, Poland\\
$ ^{29}$Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest-Magurele, Romania\\
$ ^{30}$Petersburg Nuclear Physics Institute (PNPI), Gatchina, Russia\\
$ ^{31}$Institute of Theoretical and Experimental Physics (ITEP), Moscow, Russia\\
$ ^{32}$Institute of Nuclear Physics, Moscow State University (SINP MSU), Moscow, Russia\\
$ ^{33}$Institute for Nuclear Research of the Russian Academy of Sciences (INR RAN), Moscow, Russia\\
$ ^{34}$Budker Institute of Nuclear Physics (SB RAS) and Novosibirsk State University, Novosibirsk, Russia\\
$ ^{35}$Institute for High Energy Physics (IHEP), Protvino, Russia\\
$ ^{36}$Universitat de Barcelona, Barcelona, Spain\\
$ ^{37}$Universidad de Santiago de Compostela, Santiago de Compostela, Spain\\
$ ^{38}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$ ^{39}$Ecole Polytechnique F\'{e}d\'{e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$ ^{40}$Physik-Institut, Universit\"{a}t Z\"{u}rich, Z\"{u}rich, Switzerland\\
$ ^{41}$Nikhef National Institute for Subatomic Physics, Amsterdam, The Netherlands\\
$ ^{42}$Nikhef National Institute for Subatomic Physics and VU University Amsterdam, Amsterdam, The Netherlands\\
$ ^{43}$NSC Kharkiv Institute of Physics and Technology (NSC KIPT), Kharkiv, Ukraine\\
$ ^{44}$Institute for Nuclear Research of the National Academy of Sciences (KINR), Kyiv, Ukraine\\
$ ^{45}$University of Birmingham, Birmingham, United Kingdom\\
$ ^{46}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom\\
$ ^{47}$Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom\\
$ ^{48}$Department of Physics, University of Warwick, Coventry, United Kingdom\\
$ ^{49}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$ ^{50}$School of Physics and Astronomy, University of Edinburgh, Edinburgh, United Kingdom\\
$ ^{51}$School of Physics and Astronomy, University of Glasgow, Glasgow, United Kingdom\\
$ ^{52}$Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom\\
$ ^{53}$Imperial College London, London, United Kingdom\\
$ ^{54}$School of Physics and Astronomy, University of Manchester, Manchester, United Kingdom\\
$ ^{55}$Department of Physics, University of Oxford, Oxford, United Kingdom\\
$ ^{56}$Massachusetts Institute of Technology, Cambridge, MA, United States\\
$ ^{57}$University of Cincinnati, Cincinnati, OH, United States\\
$ ^{58}$University of Maryland, College Park, MD, United States\\
$ ^{59}$Syracuse University, Syracuse, NY, United States\\
$ ^{60}$Pontif\'{i}cia Universidade Cat\'{o}lica do Rio de Janeiro (PUC-Rio), Rio de Janeiro, Brazil, associated to $^{2}$\\
$ ^{61}$Institute of Particle Physics, Central China Normal University, Wuhan, Hubei, China, associated to $^{3}$\\
$ ^{62}$Departamento de Fisica , Universidad Nacional de Colombia, Bogota, Colombia, associated to $^{8}$\\
$ ^{63}$Institut f\"{u}r Physik, Universit\"{a}t Rostock, Rostock, Germany, associated to $^{11}$\\
$ ^{64}$National Research Centre Kurchatov Institute, Moscow, Russia, associated to $^{31}$\\
$ ^{65}$Yandex School of Data Analysis, Moscow, Russia, associated to $^{31}$\\
$ ^{66}$Instituto de Fisica Corpuscular (IFIC), Universitat de Valencia-CSIC, Valencia, Spain, associated to $^{36}$\\
$ ^{67}$Van Swinderen Institute, University of Groningen, Groningen, The Netherlands, associated to $^{41}$\\
\bigskip
$ ^{a}$Universidade Federal do Tri\^{a}ngulo Mineiro (UFTM), Uberaba-MG, Brazil\\
$ ^{b}$P.N. Lebedev Physical Institute, Russian Academy of Science (LPI RAS), Moscow, Russia\\
$ ^{c}$Universit\`{a} di Bari, Bari, Italy\\
$ ^{d}$Universit\`{a} di Bologna, Bologna, Italy\\
$ ^{e}$Universit\`{a} di Cagliari, Cagliari, Italy\\
$ ^{f}$Universit\`{a} di Ferrara, Ferrara, Italy\\
$ ^{g}$Universit\`{a} di Urbino, Urbino, Italy\\
$ ^{h}$Universit\`{a} di Modena e Reggio Emilia, Modena, Italy\\
$ ^{i}$Universit\`{a} di Genova, Genova, Italy\\
$ ^{j}$Universit\`{a} di Milano Bicocca, Milano, Italy\\
$ ^{k}$Universit\`{a} di Roma Tor Vergata, Roma, Italy\\
$ ^{l}$Universit\`{a} di Roma La Sapienza, Roma, Italy\\
$ ^{m}$Universit\`{a} della Basilicata, Potenza, Italy\\
$ ^{n}$AGH - University of Science and Technology, Faculty of Computer Science, Electronics and Telecommunications, Krak\'{o}w, Poland\\
$ ^{o}$LIFAELS, La Salle, Universitat Ramon Llull, Barcelona, Spain\\
$ ^{p}$Hanoi University of Science, Hanoi, Viet Nam\\
$ ^{q}$Universit\`{a} di Padova, Padova, Italy\\
$ ^{r}$Universit\`{a} di Pisa, Pisa, Italy\\
$ ^{s}$Scuola Normale Superiore, Pisa, Italy\\
$ ^{t}$Universit\`{a} degli Studi di Milano, Milano, Italy\\
\medskip
$ ^{\dagger}$Deceased
}
\end{flushleft}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

